HICL: Hashtag-Driven In-Context Learning for Social Media Natural Language Understanding

Natural language understanding (NLU) is integral to various social media applications. However, existing NLU models rely heavily on context for semantic learning, resulting in compromised performance when faced with short and noisy social media content. To address this issue, we leverage in-context learning (ICL), wherein language models learn to make inferences by conditioning on a handful of demonstrations to enrich the context and propose a novel hashtag-driven in-context learning (HICL) framework. Concretely, we pre-train a model #Encoder, which employs #hashtags (user-annotated topic labels) to drive BERT-based pre-training through contrastive learning. Our objective here is to enable #Encoder to gain the ability to incorporate topic-related semantic information, which allows it to retrieve topic-related posts to enrich contexts and enhance social media NLU with noisy contexts. To further integrate the retrieved context with the source text, we employ a gradient-based method to identify trigger terms useful in fusing information from both sources. For empirical studies, we collected 45M tweets to set up an in-context NLU benchmark, and the experimental results on seven downstream tasks show that HICL substantially advances the previous state-of-the-art results. Furthermore, we conducted extensive analyzes and found that: (1) combining source input with a top-retrieved post from #Encoder is more effective than using semantically similar posts; (2) trigger words can largely benefit in merging context from the source and retrieved posts.

==> figure/bert-train.tex <==
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{figure/bert-train.pdf}
% % \vspace{-1em}
% \caption{\label{bert-train}
% The workflow to pre-train \#BERT on 179M Twitter posts (tweets), each containing a hashtag (left). 
% \#BERT was pre-trained on pairwise posts and contrastive learning guided them to learn topic relevance via learning to identify posts with the same hashtag (middle).
% It enables posts with the same hashtag be to pulled closer (right).
% %%and push apart those otherwise.
% %\#BERT contrastive pre-training process. \#BERT takes the tweets from the same hashtag as positive instances and other in-batch samples as negative. \#BERT target at encoding the topic and presenting embeddings which can be distinguished with respect to hashtags.
% }

% \end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{bert-train3.pdf}
% \vspace{-1em}
\caption{\label{bert-train}
The workflow to pre-train \#Retriever on 179M Twitter posts, each containing a hashtag. 
\#Retriever was pre-trained on pairwise posts and contrastive learning guided them to learn topic relevance via learning to identify posts with the same hashtag.
We randomly noise the hashtags aiming to avoid trivial representation.
%%and push apart those otherwise.
%\#BERT contrastive pre-training process. \#BERT takes the tweets from the same hashtag as positive instances and other in-batch samples as negative. \#BERT target at encoding the topic and presenting embeddings which can be distinguished with respect to hashtags.
}
\vspace{-1em}
\end{figure}

==> figure/enrich-framework.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{enrich-framework.pdf}
% \vspace{-1em}
\caption{\label{enrich-framework}
The workflow of HICL fine-tuning.
A post $\mathbf{x}$ is first encoded with \#BERT and the output is then used to search the \#Database to retrieve the most topic-related post $\mathbf{x}'$. 
After that, $\mathbf{x}'$ and $\mathbf{x}$ are paired in concatenation for task-specific fine-tuning. 
Here \#Enrich can both work for posts with and without hashtags.
%Note that source post does not required to have hashtags.
%The topic-related tweet and source tweet are then concatenated to generate a context-enriched tweet for later use.
}
\vspace{-1em}
\end{figure}
